COVID-19 incidence in the Republic of Ireland: A case study for network-based time series models

The generalised network autoregressive (GNAR) model conceptualises time series on the vertices of a network; it has an autoregressive component for temporal dependence and a spatial autoregressive component for dependence between neighbouring vertices in the network. Consequently, the choice of underlying network is essential. This paper assesses the performance of GNAR models on different networks in predicting COVID-19 cases for the 26 counties in the Republic of Ireland, over two distinct pandemic phases (restricted and unrestricted), characterised by inter-county movement restrictions. Ten static networks are constructed, in which vertices represent counties, and edges are built upon neighbourhood relations, such as railway lines. We find that a GNAR model based on the fairly sparse Economic hub network explains the data best for the restricted pandemic phase while the fairly dense 21-nearest neighbour network performs best for the unrestricted phase. Across phases, GNAR models have higher predictive accuracy than standard ARIMA models which ignore the network structure. For county-specific predictions, in pandemic phases with more lenient or no COVID-19 regulation, the network effect is not quite as pronounced. The results indicate some robustness to the precise network architecture as long as the densities of the networks are similar. An analysis of the residuals justifies the model assumptions for the restricted phase but raises questions regarding their validity for the unrestricted phase. While generally performing better than ARIMA models which ignore network effects, there is scope for further development of the GNAR model to better model complex infectious diseases, including COVID-19.

==> Sections/cover_letter.tex <==
Cover letter
Please provide a cover letter outlining your research. The cover letter should briefly discuss the context and importance of the submitted work and why it is appropriate for the journal.

Network-based time series models have experienced a surge in popularity over the past years due to their ability to model temporal and spatial dependencies, arising from the spread of infectious disease.
The generalised network autoregressive (GNAR) model conceptualises time series on the vertices of a network, for which the choice of underlying network is essential.
This paper assesses the performance of GNAR models on different networks in predicting COVID-19 cases for the 26 counties in the Republic of Ireland, over two distinct pandemic phases (restricted and unrestricted), characterised by inter-county movement restrictions.
To the best of our knowledge, the dependence of the performance of a GNAR model on the network architecture as well as its suitability to model complex infectious diseases have not been systematically explored. 
Moreover, the paper investigates network effect and its change over the duration of the pandemic. 
The paper identifies concrete research objectives for a continued development of the GNAR model.


Author declaration 
All authors wrote and reviewed the manuscript. A.S. wrote code for the data exploration and analysis.


Data availability 
Data is available on the GitHub repository for the analysis as well as on the Open Data Platform by the Government of the Republic of Ireland: https://data.gov.ie/dataset/covid-19-hpsc-county-statistics-historic-data1.


Acknowledgement 
We thank Emma Davies-Smith for insightful feedback, and Marina Knight, Guy Nason and Matt Nunes for helpful discussions.


Abstract 
Network-based time series models have experienced a surge in popularity over the past years due to their ability to model temporal and spatial dependencies, arising from the spread of infectious disease. The generalised network autoregressive (GNAR) model conceptualises time series on the vertices of a network; it has an autoregressive component for temporal dependence and a spatial autoregressive component for dependence between neighbouring vertices in the network. Consequently, the choice of underlying network is essential. This paper assesses the performance of GNAR models on different networks in predicting COVID-19 cases for the 26 counties in the Republic of Ireland, over two distinct pandemic phases (restricted and unrestricted), characterised by inter-county movement restrictions. Ten static networks are constructed, in which vertices represent counties, and edges are built upon neighbourhood relations, such as railway lines.

We find that a GNAR model based on the fairly sparse Queen's contiguity network explains the data best for the restricted pandemic phase while the fairly dense 21-nearest neighbour network performs best for the unrestricted phase. Across phases, GNAR models have higher predictive accuracy than standard ARIMA models which ignore the network structure. For county-specific predictions, in pandemic phases with more lenient or no COVID-19 regulation, the network effect is not quite as pronounced. The results indicate some robustness to the precise network architecture as long as the densities of the networks are similar. An analysis of the residuals justifies the model assumptions for the restricted phase but raises questions regarding their validity for the unrestricted phase. While outperforming ARIMA models which ignore network effects, the GNAR model warrants further development to better model complex infectious diseases, including COVID-19.
